Coding for the Gaussian Channel in the Finite Blocklength Regime Using a CNN-Autoencoder

The development of delay-sensitive applications that require ultra high reliability created an additional challenge for wireless networks. This led to Ultra-Reliable Low-Latency Communications, as a use case that 5G and beyond 5G systems must support. However, supporting low latency communications requires the use of short codes, while attaining vanishing frame error probability (FEP) requires long codes. Thus, developing codes for the finite blocklength regime (FBR) achieving certain reliability requirements is necessary. This paper investigates the potential of Convolutional Neural Networks autoencoders (CNN-AE) in approaching the theoretical maximum achievable rate over a Gaussian channel for a range of signal-to-noise ratios at a fixed blocklength and target FEP, which is a different perspective compared to existing works that explore the use of CNNs from bit-error and symbol-error rate perspectives. We explain the studied CNN-AE architecture, evaluate it numerically, and compare it to the theoretical maximum achievable rate and the achievable rates of polar coded quadrature amplitude modulation (QAM), Reed-Muller coded QAM, multilevel polar coded modulation, and a TurboAE-MOD scheme from the literature. Numerical results show that the CNN-AE outperforms these benchmark schemes and approaches the theoretical maximum rate, demonstrating the capability of CNN-AEs in learning good codes for delay-constrained applications.

==> Neural_Network.tex <==
\begin{figure}
\begin{tikzpicture}
\node (Input) at (0,0) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=blue!15, font=\small] {Input } ;

\draw [->,line width=1.5] (0 ,-0.3) --  node[pos=0.5,right,font=\small] {\footnotesize $K$ bits} (0,-0.7);

% Right brace
\draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=-2pt]
(1.5,-0.6) -- (1.5,-1.75) node [black,midway,xshift=1cm] 
{\footnotesize Encoding};

\node[] at (-1.3,-1) {$\times 3$};

\node (Conv1D_1) at (0,-1) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners, font=\small] { } ;

\node (Conv1D_2) at (0.2,-1.2) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=white, font=\small] { } ;

\node (Conv1D_3) at (0.4,-1.4) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=white, font=\small] { Conv1D} ;

\draw [->,line width=1.5] (0 ,-1.65) --  node[pos=0.28,below,font=\scriptsize] {} (0,-2.05);

\node (Reshape Layer) at (0,-2.5) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=blue!15, font=\small] {Reshape Layer } ;

\draw [->,line width=1.5] (0 ,-2.9) --  node[pos=0.28,below,font=\scriptsize] {} (0,-3.25);

\draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=-2pt]
(1.3,-3) -- (1.3,-4) node [black,midway,xshift=1.1cm] 
{\footnotesize Modulation};

\node[] at (-1.3,-3.5) {$\times 2$};

\node (Conv1D_4) at (0,-3.5) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=white, font=\small] { } ;

\node (Conv1D_5) at (0.2,-3.7) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=white, font=\small] { Conv1D} ;

\draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=-2pt]
(5,-4.5) -- (5,-3.5) node [black,midway,xshift=-1.25cm] 
{\footnotesize Demodulation};


\draw [->,line width=1.5] (0 ,-4) --  node[pos=0.55,right,align=left,font=\scriptsize,text width=1.8cm] {$n$  complex-valued symbols} (0,-4.75);

\node (Normalization Layer) at (0,-5.2) [draw,thick,align=center,text width=2cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=blue!15, font=\small] {Normalization Layer } ;

\draw [-,line width=1.5] (0 ,-5.65) --  node[pos=0.5,left,font=\small] {} (0,-6);

\draw [->,line width=1.5] (0 ,-6) --  node[pos=0.5,below,align=center,font=\small,text width=1.5cm] {$n$ complex-valued symbols} (1.86,-6);

\node (Channel) at (3,-6) [draw,thick,align=center,text width=2cm, minimum width=1.5cm,minimum height=0.5cm,rounded corners,fill=blue!15, font=\small] {Channel } ;

\draw [-,line width=1.5] (4.1 ,-6) --  node[pos=0.5,below,align=center,font=\small,text width=1.5cm] {$n$ complex-valued symbols} (5.8,-6);

\draw [->,line width=1.5] (5.8 ,-6) --  node[pos=0.28,below,font=\scriptsize] {} (5.8,-4.5);

\node[] at (7,-0.7) {$\times 3$};

\node (Conv1D_6) at (5.8,-4) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=white, font=\small] { } ;

\node (Conv1D_7) at (6,-4.2) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=white, font=\small] { Conv1D} ;
\draw [->,line width=1.5] (5.8 ,-3.75) --  node[pos=0.28,below,font=\scriptsize] {} (5.8,-2.95);

\node (Reshape Layer) at (5.8,-2.5) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=blue!15, font=\small] {Reshape Layer } ;

\draw [->,line width=1.5] (5.8 ,-2.1) --  node[pos=0.28,below,font=\scriptsize] {} (5.8,-1.65);

\draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=-2pt]
(5,-1.6) -- (5,-0.5) node [black,midway,xshift=-1cm] 
{\footnotesize Decoding};

\node[] at (7,-3.7) {$\times 2$};

\node (Conv1D_8) at (5.8,-1) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners, font=\small] { } ;

\node (Conv1D_9) at (6,-1.2) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=white, font=\small] { } ;

\node (Conv1D_10) at (6.2,-1.4) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=white, font=\small] { Conv1D} ;

\draw [->,line width=1.5] (5.8 ,-0.75) --  node[pos=0.4,right,font=\small] {\footnotesize $K$ bits} (5.8,-0.25);

\node (Output) at (5.8,0) [draw,thick,align=center,text width=1cm, minimum width=2cm,minimum height=0.5cm,rounded corners,fill=blue!15, font=\small] {Output } ;

\end{tikzpicture}
\caption{Proposed CNN-AE. The `encoding', `modulation',
`demodulation', and `decoding' layers are trained jointly.}
\label{fig:Architecture}
\end{figure}
